OATH-Frames: Characterizing Online Attitudes Towards Homelessness with LLM Assistants

Warning: Contents of this paper may be upsetting. Public attitudes towards key societal issues, expressed on online media, are of immense value in policy and reform efforts, yet challenging to understand at scale. We study one such social issue: homelessness in the U.S., by leveraging the remarkable capabilities of large language models to assist social work experts in analyzing millions of posts from Twitter. We introduce a framing typology: Online Attitudes Towards Homelessness (OATH) Frames: nine hierarchical frames capturing critiques, responses and perceptions. We release annotations with varying degrees of assistance from language models, with immense benefits in scaling: 6.5x speedup in annotation time while only incurring a 3 point F1 reduction in performance with respect to the domain experts. Our experiments demonstrate the value of modeling OATH-Frames over existing sentiment and toxicity classifiers. Our large-scale analysis with predicted OATH-Frames on 2.4M posts on homelessness reveal key trends in attitudes across states, time periods and vulnerable populations, enabling new insights on the issue. Our work provides a general framework to understand nuanced public attitudes at scale, on issues beyond homelessness.

==> figures/regression_percent.tex <==
\begin{figure}[h!]
 \includegraphics[width=0.48\textwidth]{images/regression_percent_unsheltered.pdf}
 \caption{Regression analysis: percent unsheltered and cost of living}
 \label{fig:time}
\end{figure}


==> tables/classification_metrics.tex <==


\begin{table*}[ht]
\centering
\resizebox{0.98\linewidth}{!}{
\begin{tabular}{cccccccc}
    \toprule    
    \multicolumn{8}{c}{\textbf{Aggregated (Across 9 \finer frames)}} \\
    \midrule
    \textbf{Metrics} & {\textbf{\texttt{Experts}}} & {\textbf{\gptsolo}} & {\textbf{\gptintheloop}} & {\textbf{\flanlarge}}& {\textbf{\flanbase}}& {\textbf{\flansmall}} & {\textbf{\flanxl}}\\ 
    \midrule
    {Precision} & 0.58 $\pm$ 0.08 & 0.39 $\pm$ 0.05 & 0.51 $\pm$ 0.07  & 0.54 $\pm$ 0.07 & 0.47 $\pm$ 0.06 & 0.45 $\pm$ 0.08  & 0.47 $\pm$ 0.06\\
     Recall & 0.58 $\pm$ 0.08 & 0.64 $\pm$ 0.05  & 0.6 $\pm$ 0.05 & 0.52 $\pm$ 0.05 & 0.47 $\pm$ 0.05 & 0.39 $\pm$ 0.03 & 0.55 $\pm$ 0.03 \\
      F$_1$ & 0.55 $\pm$ 0.04 & 0.46 $\pm$ 0.04 & 0.52 $\pm$ 0.04 & 0.51 $\pm$ 0.03 & 0.45 $\pm$ 0.04 & 0.38 $\pm$ 0.04 & 0.49 $\pm$ 0.03 \\
      Fleiss' $\kappa$ & 0.46 $\pm$ 0.04 & 0.31 $\pm$ 0.04  & 0.37 $\pm$ 0.04 & 0.34 $\pm$ 0.03 & 0.31 $\pm$ 0.02 & 0.24 $\pm$ 0.01 & 0.38 $\pm$ 0.04\\
    
    \bottomrule 
\end{tabular} 
}
\caption{\textbf{Macro-averaged precision, recall and F1 aggregated across all 9 \finer frames:} Comparing variations of \flan with other annotation strategies evaluated on the multiply annotated Agreement Test Set (280). }
\label{tab:res:models_vs_everyone}
\end{table*}


==> tables/flan_large_test.tex <==

\begin{table}[ht]
\centering
\resizebox{0.98\linewidth}{!}{
\begin{tabular}{ccccc}
    \toprule    
    \multicolumn{5}{c}{\textbf{Aggregated (Across 9 \finer frames)}} \\
    \midrule
    \textbf{Metrics} & {\textbf{\flanlarge}}& {\textbf{\flanbase}}& {\textbf{\flansmall}} & {\textbf{\flanxl}}\\ 
    \midrule
    {Precision} & 0.50 & 0.48 & 0.46 & 0.47\\
     Recall & 0.48 & 0.47  & 0.41 & 0.51\\
      F$_1$ & 0.50 & 0.47 & 0.42 & 0.48\\
    \bottomrule 
\end{tabular}
}
\caption{\textbf{Macro averaged precision, recall and F$_1$ on a larger test set (1280):} Comparing variations of finetuned \flan on a larger test set (1280)}
\label{tab:res:flan_models}
\end{table}



==> tables/identity_analysis.tex <==



\begin{table*}[ht]
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{p{0.25\linewidth} p{0.2\linewidth}p{0.4\linewidth}p{0.9\linewidth}}
    \toprule
    \textbf{PEH} & \textbf{Vulnerable Population}& \textbf{Significant \finer Frames}& \textbf{Example}\\ 
    \midrule
    \multirow{5}{*}{\multirowcell{18}{`Homeless' Veteran}}& \multicolumn{1}{>{\arraybackslash}p{0.2\linewidth}}{\vspace{0.5pt} Ukrainian} & \multicolumn{1}{>{\arraybackslash}p{0.4\linewidth}}{\vspace{0.5pt} \governmentcritique, \moneyaid\vspace{10pt}}& \multicolumn{1}{>{\arraybackslash}p{0.9\linewidth}}{\vspace{0.01pt} {\fontfamily{cmss}\selectfont @mention they have been given not 1 billon dollars, not 80 billion dollars (russian military budgets, but 180 billion dollars. do you really think that money is being used to help the ukrainian people-or is it something else? go help a homeless vet today!} \newline \textbf{Post labeled with: }\moneyaid, \governmentcritique, \deservingundeserving\vspace{10pt}} \\\cline{2-4}
    
                        & \multicolumn{1}{>{\arraybackslash}p{0.2\linewidth}}{\vspace{0.5pt} Illegal Alien} & \multicolumn{1}{>{\arraybackslash}p{0.4\linewidth}}{\vspace{0.5pt} \governmentcritique, \personalinteraction, \mediaportrayal, \nimby\vspace{10pt}}& \multicolumn{1}{>{\arraybackslash}p{0.9\linewidth}}{\vspace{0.01pt} {\fontfamily{cmss}\selectfont and this is being done for your homeless, especially homeless veterans, on your city streets? no? well? i didn't think so. send the illegal aliens back to where they came from! vote red!} \newline \textbf{Post labeled with: }\governmentcritique, \nimby, \deservingundeserving\vspace{10pt}} \\\cline{2-4}
                        
                        & \multicolumn{1}{>{\arraybackslash}p{0.2\linewidth}}{\vspace{0.5pt} Asylum Seeker} & \multicolumn{1}{>{\arraybackslash}p{0.4\linewidth}}{\vspace{0.5pt} \societalcritique, \solutionsinterventions, \personalinteraction, \mediaportrayal, \nimby, \harmfulgeneralization\vspace{10pt}}& \multicolumn{1}{>{\arraybackslash}p{0.9\linewidth}}{\vspace{0.01pt} {\fontfamily{cmss}\selectfont @mention better still, if you’re so concerned for homeless veterans get off your soapbox and go volunteer to help them. they won’t be blaming asylum seekers for their situation. and maybe while you’re at it, try meeting an asylum seeker….\#spreadinghatethroughignorance} \newline \textbf{Post labeled with: }\societalcritique, \solutionsinterventions, \deservingundeserving\vspace{10pt}} \\\cline{2-4}
                        
                        & \multicolumn{1}{>{\arraybackslash}p{0.2\linewidth}}{\vspace{0.5pt} Refugee} & \multicolumn{1}{>{\arraybackslash}p{0.4\linewidth}}{\vspace{0.5pt} \societalcritique, \solutionsinterventions, \harmfulgeneralization\vspace{10pt}}& \multicolumn{1}{>{\arraybackslash}p{0.9\linewidth}}{\vspace{0.01pt} {\fontfamily{cmss}\selectfont @mention typical american who never travels unless on a cruise ship or american! asia is amazing \&amp; for someone who is the daughter of a disabled refugee/ don’t lecture me on not respecting our amazing veterans. at least we take care of then here - how many millions of homeless vets in us?} \newline \textbf{Post labeled with: }\societalcritique \deservingundeserving\vspace{10pt}} \\\cline{2-4}
                        
                        & \multicolumn{1}{>{\arraybackslash}p{0.2\linewidth}}{\vspace{0.5pt} Immigrant} & \multicolumn{1}{>{\arraybackslash}p{0.4\linewidth}}{\vspace{0.5pt}\nimby\vspace{10pt}}& \multicolumn{1}{>{\arraybackslash}p{0.9\linewidth}}{\vspace{0.01pt} {\fontfamily{cmss}\selectfont @mention oh please they are dropping off bus loads of immigrants to hotels 6 blocks from my house that we the tax payers get to pay for. we have homeless vets what about them !! wake up} \newline \textbf{Post labeled with: }\nimby, \governmentcritique, \deservingundeserving\vspace{10pt}} \\ \midrule 



                        
    \multirow{5}{*}{\multirowcell{18}{`Homeless' People}}& \multicolumn{1}{>{\arraybackslash}p{0.2\linewidth}}{\vspace{0.5pt} Ukrainian} & \multicolumn{1}{>{\arraybackslash}p{0.4\linewidth}}{\vspace{0.5pt} \governmentcritique, \moneyaid\vspace{10pt}}& \multicolumn{1}{>{\arraybackslash}p{0.9\linewidth}}{\vspace{0.01pt} {\fontfamily{cmss}\selectfont ukrainian refugees can get ssi, housing benefits, and free health care. meanwhile, we have a lot of homeless people who have no access to such benefits - we have the highest number of the unemployed black population.} \newline \textbf{Post labeled with: }\moneyaid, \governmentcritique, \deservingundeserving\vspace{10pt}} \\\cline{2-4}
    
                        & \multicolumn{1}{>{\arraybackslash}p{0.2\linewidth}}{\vspace{0.5pt} Illegal Alien} & \multicolumn{1}{>{\arraybackslash}p{0.4\linewidth}}{\vspace{0.5pt} \governmentcritique, \nimby, \harmfulgeneralization\vspace{10pt}}& \multicolumn{1}{>{\arraybackslash}p{0.9\linewidth}}{\vspace{0.01pt} {\fontfamily{cmss}\selectfont @mention when adams was sworn into office, there were already an estimated 1/2 million illegal aliens in nyc. it hasn't been reported yet, whether or not adams has continued the deblasio \&amp; bloomberg policy of shipping homeless people outside of nyc, as a cheaper option than sheltering.} \newline \textbf{Post labeled with: }\nimby, \governmentcritique, \deservingundeserving\vspace{10pt}} \\\cline{2-4}

                        
                        & \multicolumn{1}{>{\arraybackslash}p{0.2\linewidth}}{\vspace{0.5pt} Asylum Seeker} & \multicolumn{1}{>{\arraybackslash}p{0.4\linewidth}}{\vspace{0.5pt} \societalcritique, \solutionsinterventions, \mediaportrayal, \harmfulgeneralization\vspace{10pt}}& \multicolumn{1}{>{\arraybackslash}p{0.9\linewidth}}{\vspace{0.01pt} {\fontfamily{cmss}\selectfont @mention i take it you’ll be taking your colleagues to task then if they slam those on welfare ? maybe; just maybe , you could support both homeless people and asylum seekers . i know that’s a hard one for you to understand.} \newline \textbf{Post labeled with: }\solutionsinterventions, \societalcritique, \deservingundeserving\vspace{10pt}} \\\cline{2-4}

                        
                        & \multicolumn{1}{>{\arraybackslash}p{0.2\linewidth}}{\vspace{0.5pt} Refugee} & \multicolumn{1}{>{\arraybackslash}p{0.4\linewidth}}{\vspace{0.5pt} \societalcritique, \solutionsinterventions, \mediaportrayal\vspace{10pt}}& \multicolumn{1}{>{\arraybackslash}p{0.9\linewidth}}{\vspace{0.01pt}{\fontfamily{cmss}\selectfont @mention refugee camps offer a safe haven for refugees and meet their most basic needs such as food water shelter medical treatment and other basic services there are homeless people all over america that don't even get that..yeah sorry but hater @mention bad sad story been played out \#btc} \newline \textbf{Post labeled with: }\societalcritique, \solutionsinterventions, \deservingundeserving\vspace{10pt}} \\\cline{2-4}

                        
                        & \multicolumn{1}{>{\arraybackslash}p{0.2\linewidth}}{\vspace{0.5pt} Immigrant} & \multicolumn{1}{>{\arraybackslash}p{0.4\linewidth}}{\vspace{0.5pt}\personalinteraction, \nimby, \harmfulgeneralization\vspace{10pt}}& \multicolumn{1}{>{\arraybackslash}p{0.9\linewidth}}{\vspace{0.01pt} {\fontfamily{cmss}\selectfont @mention new york city’s pulling the rug out from underneath the illegal immigrants kicking them out of the \$700 a day hotel rooms. was it the bedbugs or the thousands of empty bottles of beer and liquor. we used to have a problem with homeless people now we have a catastrophe of homeless} \newline \textbf{Post labeled with: }\nimby, \governmentcritique, \deservingundeserving\vspace{10pt}} \\ \midrule


\multirow{5}{*}{\multirowcell{18}{`Homeless' American}}& \multicolumn{1}{>{\arraybackslash}p{0.2\linewidth}}{\vspace{0.5pt} Ukrainian} & \multicolumn{1}{>{\arraybackslash}p{0.4\linewidth}}{\vspace{0.5pt} \governmentcritique, \moneyaid\vspace{10pt}}& \multicolumn{1}{>{\arraybackslash}p{0.9\linewidth}}{\vspace{0.01pt} {\fontfamily{cmss}\selectfont @mention grifter journalist got to grift . how about reporting on how close we are from being in a nuclearwar with russia. or how corrupted our politicians have become. write about how homeless americans live across this country and the us thinks sending money to ukraine is saving anyone} \newline \textbf{Post labeled with: }\moneyaid, \governmentcritique, \deservingundeserving\vspace{10pt}} \\\cline{2-4}

     
                        & \multicolumn{1}{>{\arraybackslash}p{0.2\linewidth}}{\vspace{0.5pt} Illegal Alien} & \multicolumn{1}{>{\arraybackslash}p{0.4\linewidth}}{\vspace{0.5pt} \governmentcritique, \nimby, \harmfulgeneralization\vspace{10pt}}& \multicolumn{1}{>{\arraybackslash}p{0.9\linewidth}}{\vspace{0.01pt}{\fontfamily{cmss}\selectfont @mention i say bus the illegal aliens to the places where the homeless americans and veterans are freezing outside.  that way our homeless citizens might get some of their tax resources back by being mistaken for illegal aliens or (lol) migrants.} \newline \textbf{Post labeled with: }\nimby, \governmentcritique, \deservingundeserving\vspace{10pt}}\\\cline{2-4}

                        
                        & \multicolumn{1}{>{\arraybackslash}p{0.2\linewidth}}{\vspace{0.5pt} Asylum Seeker} & \multicolumn{1}{>{\arraybackslash}p{0.4\linewidth}}{\vspace{0.5pt} \societalcritique, \solutionsinterventions, \harmfulgeneralization\vspace{10pt}}& \multicolumn{1}{>{\arraybackslash}p{0.9\linewidth}}{\vspace{0.01pt}{\fontfamily{cmss}\selectfont @mention hey there are plenty of homeless americans where is the welcome committee for them?!! you don’t care about being  a “ humanitarian “ or you would start by those who have birth rights in the usa not false claims to asylum… you people are pathetic..\#clownsagenda} \newline \textbf{Post labeled with: }\societalcritique, \solutionsinterventions, \deservingundeserving\vspace{10pt}}\\\cline{2-4}


                        
                        & \multicolumn{1}{>{\arraybackslash}p{0.2\linewidth}}{\vspace{0.5pt} Refugee} & \multicolumn{1}{>{\arraybackslash}p{0.4\linewidth}}{\vspace{0.5pt} \societalcritique, \solutionsinterventions, \personalinteraction, \mediaportrayal\vspace{10pt}}& \multicolumn{1}{>{\arraybackslash}p{0.9\linewidth}}{\vspace{0.01pt}{\fontfamily{cmss}\selectfont @mention see there you go avoiding the question, can't ask me to play semantics with you if you won't reciprocate. you got one spot left, a homeless american or fresh new refugee, who gets helped first. if you say at the same time then you are just avoiding your own hard truth} \newline \textbf{Post labeled with: }\societalcritique, \solutionsinterventions, \deservingundeserving\vspace{10pt}} \\\cline{2-4}


                        
                        & \multicolumn{1}{>{\arraybackslash}p{0.2\linewidth}}{\vspace{0.5pt} Immigrant} & \multicolumn{1}{>{\arraybackslash}p{0.4\linewidth}}{\vspace{0.5pt}\societalcritique, \solutionsinterventions, \personalinteraction, \mediaportrayal, \nimby, \harmfulgeneralization\vspace{10pt}}&\multicolumn{1}{>{\arraybackslash}p{0.9\linewidth}}{\vspace{0.01pt}{\fontfamily{cmss}\selectfont @mention well... if we didn't have all the illegals here. maybe we could actually get a handle on homeless americans. problem solved. what's your solution? just empty platitudes.} \newline \textbf{Post labeled with: }\societalcritique, \solutionsinterventions, \deservingundeserving\vspace{10pt}} \\
    \bottomrule 
\end{tabular}
}
\caption{Statistically significant frames for posts containing (PEH, Vulnerable Population) co-occurrence pairs.}
\label{tab:appendix:identity_full}
\end{table*}





==> tables/solutions_examples.tex <==

\begin{table}[ht]
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{p{0.4\linewidth} p{0.99\linewidth}}
    \toprule
    \textbf{(State, Attitude)} & \textbf{Post}\\ 
    \midrule
    (New York, \moneyaid) & {\fontfamily{cmss}\selectfont  how much,money is allotted to illegal migrants? do you know? they sure are trashing out new york. everywhere they congregate there's piles of trash. how dare them through food away when we have so many homeless americans! funds need to help our people first!} \\
     \midrule
    (New York, \deservingundeserving) & {\fontfamily{cmss}\selectfont you’re right.  we should be feeding and housing our homeless veterans with our tax dollars instead of housing ungrateful illiberal immigrants in nyc high rises.  also - pay your own debt.} \\
    \midrule
    (California, \societalcritique) & {\fontfamily{cmss}\selectfont you idiots , help our homeless people first , help people in california that can’t even find food or clothes.} \\
     \midrule
    (California, \harmfulgeneralization) & {\fontfamily{cmss}\selectfont talk about how california has been ruined under you! los angeles and san francisco used to be wonderful, safe, clean cities! now they’re packed with homeless, drug addicts, violent lunatics, car thieves, murderers, and more. you’re a vile pig!} \\
   \midrule
    (Florida, \mediaportrayal) & {\fontfamily{cmss}\selectfont google alexia son peter. he absolutely beat the shit out of a homeless man on season 3. he’s also beat up his girlfriend. also he never even went to university of miami and is not allowed to be there.} \\
     \midrule
    (Oregon, \harmfulgeneralization) & {\fontfamily{cmss}\selectfont portland street response is a joke, i’m sorry.  the majority of the homeless who come to portland aren’t from here and likely to be criminals. have you missed the amount of fentanyl being dealt and the amount of guns within the homeless population?} \\
    \bottomrule 
\end{tabular}
}
\caption{\textbf{Examples of posts containing mentions San Francisco or Los Angeles labeled with \solutionsinterventions.}
\label{tab:solutions_examples}
\end{table}


==> tables/tab-frames_examples.tex <==
\begin{table*}[t]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}llc@{}}
\multicolumn{1}{c}{\textbf{Core Frame}} & \multicolumn{1}{c}{\textbf{Tweet}} & \multicolumn{1}{c}{\textbf{Human Annotations}}  \\ \toprule
Critique & \begin{tabular}[c]{@{}l@{}l@{}}\textit{@REPLY how does someone who can't solve the homeless issues,} \\ \textit{crime issues and imposes mandates on others except his family,have the nerves} \\ \textit{to talk about what another state is doing? take care of your state's problems sir!}\end{tabular}
& \texttt{<made\_an\_example>, <government\_critique> }\\ \rowcolor{gray!15} 
 & \begin{tabular}[c]{@{}l@{}l@{}}\textit{some christian you are... filming these poor homeless people and callously} \\  \textit{putting them out there while saying another group of people should} \\ \textit{just go die by the hand of basically the anti christ}\end{tabular} & \texttt{<performative\_activism>, <societal\_critique> }\\
 & \begin{tabular}[c]{@{}l@{}l@{}l@{}}\textit{i love soccer and kansas city but dude no one wants that new stadium built} \\ \textit{over the river front park. use that money to clean up the fucking city,} \\ \textit{it’s disgusting. help the homeless with that stadium money. i’m so} \\ \texit{sick of seeing more trash and more homeless people every damn year} \end{tabular}
 & \texttt{<money\_aid\_resource\_allocation>}\\ \rowcolor{gray!15} \hline
\cellcolor{white} Response to  & \begin{tabular}[c]{@{}l@{}l@{}}\textit{@REPLY They were just taking from the rich and feeding the } \\ \textit{homeless... I hear that's tradition in Nottingham } \\ \textit{when the Sherriff isn't around to stop it.} \end{tabular}
& \texttt{<civic\_engagement>} \\ 
 \cellcolor{white} homelessness & \begin{tabular}[c]{@{}l@{}l@{}}\textit{\textit{@REPLY I think all homeless people should go to Ottawa and protest to our Government}} \\ \textit{ about the horrible conditions they live with. Being arrested might be better then their } \\ \textit{current conditions at least they’ll have a bed and 3 meals per day.What do you think Evan???????} \end{tabular}  & \texttt{<call\_to\_action>,<solutions\_interventions>}\\ \rowcolor{gray!15}
 & \begin{tabular}[c]{@{}l@{}}\textit{@REPLY Did you guys catch and kill that homeless person } \\ \textit{who burned down your metal Christmas tree yet?.} \end{tabular}
  & \texttt{<violence\_against\_PEH>}\\  \hline
 \cellcolor{white} Perceptions \&  & \begin{tabular}[c]{@{}l@{}l@{}}\textit{@REPLY too little too late. with all those illegal aliens coming into your crime ridden} \\ \textit{city, the homeless population will be sleeping in snowbanks this winter.} \\ \textit{you and your city council are all about to be impeached.} \end{tabular}
& \texttt{<anti\_immigration>, <deserving\_undeserving>} \\ \rowcolor{gray!15}
 \cellcolor{white} Discrimination & \textit{@REPLY take your 3k homeless sidewalk defecating followers and eat me} & \texttt{<dehumanizing>,<harmful\_generalization>} \\ 
 \cellcolor{white} of PEH & \begin{tabular}[c]{@{}l@{}l@{}}\textit{@REPLY Imagine this now and I am not voting until 2026. Let’s fucking go.} \\ \textit{  You need to come and see the streets in Downtown, full of homeless.} \\ \textit{The worst? 2nd Avenue. I am glad I live in Broward} \end{tabular}
  & \texttt{<not\_in\_my\_backyard>,<personal\_interaction\_observation\_of\_homelessness>}\\ 
 \bottomrule
\end{tabular}%
}
\caption{Examples of tweets from each core frame, and corresponding human annotations selected from finer-grained labels}
\label{tab:frames_examples}
\end{table*}
